Subtle Signals: Video-based Detection of Infant Non-nutritive Sucking as a Neurodevelopmental Cue

Non-nutritive sucking (NNS), which refers to the act of sucking on a pacifier, finger, or similar object without nutrient intake, plays a crucial role in assessing healthy early development. In the case of preterm infants, NNS behavior is a key component in determining their readiness for feeding. In older infants, the characteristics of NNS behavior offer valuable insights into neural and motor development. Additionally, NNS activity has been proposed as a potential safeguard against sudden infant death syndrome (SIDS). However, the clinical application of NNS assessment is currently hindered by labor-intensive and subjective finger-in-mouth evaluations. Consequently, researchers often resort to expensive pressure transducers for objective NNS signal measurement. To enhance the accessibility and reliability of NNS signal monitoring for both clinicians and researchers, we introduce a vision-based algorithm designed for non-contact detection of NNS activity using baby monitor footage in natural settings. Our approach involves a comprehensive exploration of optical flow and temporal convolutional networks, enabling the detection and amplification of subtle infant-sucking signals. We successfully classify short video clips of uniform length into NNS and non-NNS periods. Furthermore, we investigate manual and learning-based techniques to piece together local classification results, facilitating the segmentation of longer mixed-activity videos into NNS and non-NNS segments of varying duration. Our research introduces two novel datasets of annotated infant videos, including one sourced from our clinical study featuring 19 infant subjects and 183 hours of overnight baby monitor footage.

==> difference.tex <==
1. The journal introduces the challenging NNS data which has NNS overwhelmed by the background action noise. Corresponding action recognition evaluations are carefully elaborated.

2. Newly introduced end-to-end deep-learning-based action segmentation model.

3. An exhaustive experimental comparison of our method with various spatiotemporal models.



==> highlight.tex <==
1. NNS Action Recognition and Segmentation: The technical contributions of this work address both fine-grained NNS action recognition and broader NNS action segmentation challenges. The former involves classifying 2.5-second video clips as NNS or non-NNS, while the latter identifies frames with NNS activity in minute-long video clips. These tasks are accomplished using convolutional long short-term memory networks and local NNS recognition with sliding windows.

2. Data Creation: The paper introduces two new datasets: the "NNS clinical in-crib dataset" comprising nighttime in-crib baby monitor footage from 19 infants, manually annotated for NNS activity, and the "NNS in-the-wild dataset" consisting of naturalistic infant video clips annotated for NNS activity. These datasets include challenging conditions and infant poses, enhancing the diversity of available data.

3. Methodological Enhancements: The research presents a comprehensive NNS classification system that employs convolutional long short-term memory networks. This system is supported by domain-specific infant face localization, video stabilization, and customized signal enhancement techniques. The paper also includes new performance evaluations on a challenging dataset to validate the method's effectiveness.

4. Experimental Comparison: The article conducts an exhaustive experimental comparison of their approach with various spatiotemporal models, emphasizing its performance and effectiveness in NNS detection and segmentation tasks.
